Advanced Equalization in 112 Gb/s Upstream PON Using a Novel Fourier Convolution-based Network

We experimentally demonstrate a novel, low-complexity Fourier Convolution-based Network (FConvNet) based equalizer for 112 Gb/s upstream PAM4-PON. At a BER of 0.005, FConvNet enhances the receiver sensitivity by 2 and 1 dB compared to a 51-tap Sato equalizer and benchmark machine learning algorithms respectively.

==> tables/tab1.tex <==
% \begin{center}
% \begin{table*}[t]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lllllllll}
% \hline
% \textbf{dBm}    & \textbf{TimesNet (wl=512)} & \textbf{TimesNet (wl=256)} & \textbf{FC-SCINet} & \textbf{Dlinear} & \textbf{DNN (2-layer)} & \textbf{DNN (3-layer)} & \textbf{Linear+CNN} & \textbf{Baseline} \\ \hline

% \textbf{-6dbm}  & 1.239e-03                  & 1.362e-03                  & 2.366e-03          & 6.103e-03        & 2.018e-03              & 2.131e-03              & 2.282e-03           & 3.944e-03         \\ %\hline
% \textbf{-7dbm}  & 1.550e-03                  & 1.794e-03                  & 2.882e-03          & 6.591e-03        & 2.498e-03              & 2.451e-03              & 2.713e-03           & 4.301e-03         \\ %\hline
% \textbf{-8dbm}  & 2.329e-03                  & 2.620e-03                  & 3.934e-03          & 7.661e-03        & 3.643e-03              & 3.728e-03              & 3.596e-03           & 5.032e-03         \\ %\hline
% \textbf{-9dbm}  & 3.794e-03                  & 4.000e-03                  & 5.653e-03          & 9.776e-03        & 5.812e-03              & 5.606e-03              & 5.362e-03           & 5.961e-03         \\ %\hline
% \textbf{-10dbm} & 5.370e-03                  & 5.624e-03                  & 7.399e-03          & 1.151e-02        & 7.267e-03              & 7.342e-03              & 7.624e-03           & 7.566e-03         \\ %\hline
% \textbf{-11dbm} & 8.936e-03                  & 9.120e-03                  & 1.087e-02          & 1.507e-02        & 1.087e-02              & 1.078e-02              & 1.114e-02           & 1.048e-02         \\ %\hline
% \textbf{-12dbm} & 1.401e-02                  & 1.423e-02                  & 1.640e-02          & 2.230e-02        & 1.690e-02              & 1.650e-02              & 1.741e-02           & 1.374e-02         \\ \hline
% \textbf{Improvement \%} & 68.4\% & 58.5\% & 40.8\% & 65.6\% & 47.1\% & 45.2\% & 39.6\% & 0\% \\ \hline
% \end{tabular}%
% }
% \end{table*}
% \end{center}

==> tables/tab2.tex <==
% \begin{center}
%   \begin{table*}[t]
%     \centering
%     \captionsetup{font=footnotesize}
%     \footnotesize
%     \setlength{\tabcolsep}{5pt}
%     \renewcommand{\arraystretch}{1.2} 
%     \caption{Comparison of RMpS, mBER, and PRB}
%     \begin{tabular}{lccc}
%       \toprule
%       \vspace{-2pt}
%       Model & RMpS(Value) & mBER & PRB \\
%       \midrule
%       \vspace{-2pt}
%       DNN &  209,700 & 0.089912 & 18854.55 \\
%       CNN &  209,700 & 0.089912 & 18854.55 \\
%       FC-SCINet &  187,520 & 0.000071& 13.31 \\
%       FConvNet & $ (n_{i} \cdot n_{k} \cdot n_{f}) \cdot \left(\frac{n_{s}+2 \cdot \text{padding} - \text{dilation} \cdot (n_{k} - 1) - 1}{\text{stride}} + 1\right)
% $ & $ \text{todo} $ & $ \text{todo} $ \\
%       \bottomrule
%     \end{tabular}
%     \label{tab:tab2}
%   \end{table*}
% \end{center}

